White-box Testing of NLP models with Mask Neuron Coverage

Recent literature has seen growing interest in using black-box strategies like CheckList for testing the behavior of NLP models. Research on white-box testing has developed a number of methods for evaluating how thoroughly the internal behavior of deep models is tested, but they are not applicable to NLP models. We propose a set of white-box testing methods that are customized for transformer-based NLP models. These include Mask Neuron Coverage (MNCOVER) that measures how thoroughly the attention layers in models are exercised during testing. We show that MNCOVER can refine testing suites generated by CheckList by substantially reduce them in size, for more than 60\% on average, while retaining failing tests -- thereby concentrating the fault detection power of the test suite. Further we show how MNCOVER can be used to guide CheckList input generation, evaluate alternative NLP testing methods, and drive data augmentation to improve accuracy.

==> MoreText.tex <==
Recent literature pointed out that additional evalua- tion metrics are necessary to make deep NLP systems suitable for high-security domains like medicine or legal applications. This includes evaluating robustness for noise [6, 96], adversarial changes [93, 40], fairness [86], logical consistency [90], explanations [91], diagnostic datasets [122], and interactive error analysis [126]. This proposal focuses on the adversarial robustness.Connecting Adversarial Examples to Property Validation in Software Testing for DNN. Software testing refers to any activity that aims to detect the differences between existing and required property (i.e., property validation) [4]. Software testing provides effective tools to increase the user’s confidence in the correctness of a software via validating properties that its users care. Recently many software engineering techniques have been adapted to generate test inputs for validating properties of DNNs, including symbolic execution [112, 30], metamorphic testing [9], fuzz testing [31], combinatorial testing [70], and abstract interpretation [71]. Software testing techniques require a test suite (e.g., a set of inputs), an oracle (e.g., answers to each test input) and criteria that defines the adequacy requirements of test cases. ”Test input generation,” is a sub-field in software testing and is closely related to the research topics of adversarial example generation.Trustworthiness builds through Property Validation and Interpretations. Huang et al. [39] defined the process of checking trustworthiness of DNN models as to address two processes: a property validation process and an explanation process. The property validation process is held before the deployment of the model to ensure that it functions correctly with respect to a set of property requirements. The explanation process is held whenever needed during the lifetime of model deployment. In other words, a user is able to trust a system if the system has been validated, any of its behaviour can be well explained and the interpretations are not fragile.Adversarial examples expose regions of the input space where learning models perform poorly, therefore such studies can aid in understanding and im- proving deep learning in NLP. This proposal aim to build a comprehensive benchmark framework for adversarial robustness in deep NLP.Multiple recent works have focused on applying the concept of adversarial examples to text, including [3, 52, 57, 136, 21, 25, 61, 97, 62, 49, 41, 84]. These attacks on text adversarial examples all tried to generate modifications to transform x to x′ and make that modification hard to detect, and xadv is mostly generated via an iterative process involving many middle step x′. They differ with regards to how they conduct the transformation and how to define the distance between x and x′ (Figure 2 shows exemplar transformations that modify one discrete sequence x to another discrete x′; ). (1) Attacks by Character Substitution [21, 25, 61]; (2) Attacks by Paraphrase [94, 41]; (c) Attacks by Synonym Substitution [3, 52, 57, 84]; (d) Attacks by Word Insertion or Removal [62, 97]; (e) Attack by limiting Lp distance in a latent embedding space [138].We, therefore, propose to design new attacks and add re- implementation of existing literature to go beyond one input structure, namely word or characters. There exist many possible ways to expand the transformation space.The ground-breaking Transformer ar- chitectures have facilitated building higher-capacity NLP models via a unified set of APIs and pretraining has made it possible to effectively utilize this capacity for a wide variety of tasks. The Hugging Face Transformers open-source library includes a curated collection of pretrained models covering more than hundreds of different languages [125]. Essentially, we can treat ”text adversarial examples” as a special group of test inputs that follow metamorphic relations defined by language constraints, and at the same time result in fragile predictions or fragile interpretations. Such a redefinition enables us to use those ”test adequacy criterion” defined in the literature to answer that question on ”have we generated enough for checking the adversarial robustness?”. Most coverage measures in the testing literature have not been explored for deep NLP yet, especially when focusing on text adversarial examples generations.Next, we will design a workflow using the proposed coverage metrics, to guide adversarial text sample generation (to maximize coverage). Our workflow aims to achieve both intensive testing (i.e., non-trivial to achieve high coverage) and computational feasibility (by incorporating the cost analysis from Task 3b). We propose to investigate how to select proper transformations for generating sample sets with a better coverage. Further, we will benchmark the previous proposed coverage metrics for DNNs against our proposed when applied to NLP models.





\fix{above intro is more for testing focused}
\plan{NLP INTRO ALTERNATIVE: }

\plan{what does coverage measure?} We define a test set sequence $T= [t_1, \dots, t_N]$ \fix{and let $t_c$ be the point where we achieve MaxCover.}  and $\theta \in R^L$ are the parameters of the `test' neural network. \fix{$t_c$, this should be independent of order?, its independent if taken in the combinatorial sense, otherwise highly dependent on chosen test sequence, seems close to density estimation using vector quantization}  \fix{ this is a relationship between input space $R^M$ and model space $R^L$, $t$ defines both a point in $R^M$ and $R^L$}. $C(\theta,T): R^L \rightarrow R = f([\mathbf{C}_1, \dots, \mathbf{C}_N]) \mathbf{C}_t \in R^L$. Here, $\mathbf{C}_t : R^M \rightarrow R^L$. We assume an inverse mapping $\mathbf{C}^{-1}_t : R^L \rightarrow R^M$.  We denote $q_{\theta}(C_t)$ as the distribution of $C_t$ under network $\theta$. There are two distances here $q_{\theta}(C_t)$ and $p_{\theta}(X)$ as well as $p_{\theta}(X)$ and $p(X)$.  Maximizing coverage for a sample, $c \in R^L$, aims to surprise $q_{\theta}(c)$. Constraint should be added $\mathbf{C}^{-1}_t(c) \sim p(X)$   .Coverage $C(\theta,T)$,  measures the extent to which the space defined by the finite test set $T$, $H(T)\in \mathbb{R}^M$, where $T$ is a given set of test data and , approximates the   $p_{\theta}(X)$ \fix{$q_{\theta}(C_t)$???$p_{\theta}(X,Y)$???} distribution. 

\plan{}

\fix{coverage is used to guide test set generation, we still need a transformation function. For now using TextFooler, with goal function untargeted classification? as well as coverage maximization, basically make new attack recipe with goal function as MaxCoverage}
Why? Test techniques that generate large number of inputs without being important for testing the functional logic of the DNN or diversity, increase cost with little value. After training, DNNs either use natural inputs or adversarial inputs for testing. 
 
 The effectiveness of these methods has been checked using accuracy measurements on a test set. However, these do not help uncover errors or do not reveal ``bugs" in the DNN computation model. Recent work\cite{checklist:acl20} has tried to find these errors or potential sources of bugs using hand designed rules. Differently, studies in software testing have explored using coverage based methods to generate such error cases automatically.  Maximizing the coverage closely relates to generating adversarial samples\fix{they show gradient is the same}\cite{li2019structural}.



Coverage in software engineering, is a test adequacy measure, used to measure how adequate or complete a putative ``test set" is\cite{horgan1994achieving}. This is a requirement for a program to be deemed bug-free or safe. Another category is Mutation Testing. Test adequacy criterion is a predicate
that defines “what properties of a program must be exercised to constitute a
‘thorough’ test, i.e., one whose successful execution implies no errors in a
tested program\cite{zhu1997software}. Simply put, by adequacy, we mean we have checked a good amount of corner cases (where the model may misbehave) and can used the failed cases to see where the model fails. 

Mathematically: $C(f, T)$, coverage is a function of the set $T$ and the function $f$. 
In most DNN testing studies, errors are defined as:
\begin{itemize}
    \item Adversarial Samples
    \item Natural Inputs that are misclassified
\end{itemize}


Adversarial samples are classed as bugs or errors in a DNN.  Why does this work for a regular DNNs? 
\fix{Under what cases is neuron coverage a good method of generating adversarial samples?}
Compared to the pre-training process, enhancing the fine-tuning process is less timeconsuming and can better adapt to downstream
tasks.





==> sentiment_table.tex <==

\multirow{10}{*}{\rotatebox[origin=c]{90}{Vocab.+POS}}
& \textbf{\em MFT:} Short sentences with neutral adjectives and nouns & 0.0 & 7.6 & 4.8 & 94.6 & 81.8 & \makecell[ml]{\example{The company is Australian.}{\neutral} \\\example{That is a private aircraft.}{\neutral}} \\
\addlinespace
& \textbf{\em MFT:} Short sentences with sentiment-laden adjectives & 4.0 & 15.0 & 2.8 & 0.0 & 0.2 & \makecell[ml]{\example{That cabin crew is extraordinary.}{\pos} \\\example{I despised that aircraft.}{\neg}} \\
\addlinespace
& \textbf{\em INV:} Replace neutral words with other neutral words & 9.4 & 16.2 & 12.4 & 10.2 & 10.2 & \makecell[ml]{\example{@Virgin should I be concerned \swap{that}{when} I'm about to fly ...}{\inv} \\\example{@united \swap{the}{our} nightmare continues...}{\inv}} \\ %
\addlinespace
& \textbf{\em DIR:} Add positive phrases, fails if sent. goes down by $> 0.1$ &12.6 & 12.4 & 1.4 & 0.2 & 10.2 & \makecell[ml]{\example{@SouthwestAir Great trip on 2672 yesterday... \add{You are extraordinary.}}{\up} \\\example{@AmericanAir AA45 ... JFK to LAS. \add{You are brilliant.}}{\up}} \\ & \textbf{\em DIR:} Add negative phrases, fails if sent. goes up by $> 0.1$ & 0.8 & 34.6 & 5.0 & 0.0 & 13.2& \makecell[ml]{\example{@USAirways your service sucks. \add{You are lame.}}{\down} \\\example{@JetBlue all day. \add{I abhor you.}}{\down}} \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{0}{Robust.}}
& \textbf{\em INV:} Add randomly generated URLs and handles to tweets & 9.6 & 13.4 & 24.8 & 11.4 & 7.4 & \makecell[ml]{\example{@JetBlue that selfie was extreme. \add{@pi9QDK}}{\inv} \\\example{@united stuck because staff took a break? Not happy 1K.... \add{https://t.co/PWK1jb}}{\inv}} \\
\addlinespace
& \textbf{\em INV:} Swap one character with its neighbor (typo)& 5.6 & 10.2 & 10.4 & 5.2 & 3.8& \makecell[ml]{\example{\swap{@JetBlue}{@JeBtlue} I cri}{\inv} \\\example{@SouthwestAir no \swap{thanks}{thakns}}{\inv}} \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{NER}}
& \textbf{\em INV:} Switching locations should not change predictions & 7.0 & 20.8 & 14.8 & 7.6 & 6.4& \makecell[ml]{\example{@JetBlue I want you guys to be the first to fly to \#\swap{Cuba}{Canada}...}{\inv} \\\example{@VirginAmerica I miss the \#nerdbird in \swap{San Jose}{Denver}}{\inv}} \\
\addlinespace
& \textbf{\em INV:} Switching person names should not change predictions & 2.4 & 15.1 & 9.1 & 6.6 & 2.4 & \makecell[ml]{\example{
...Airport agents were horrendous. \swap{Sharon}{Erin} was your saviour}{\inv}
 \\\example{@united 8602947, \swap{Jon}{Sean} at http://t.co/58tuTgli0D, thanks.}{\inv}} \\
\midrule
\multirow{1}{*}{\rotatebox[origin=c]{0}{Temporal}}
& \textbf{\em MFT:} Sentiment change over time, present should prevail &41.0 & 36.6 & 42.2 & 18.8 & 11.0  & \makecell[ml]{\example{I used to hate this airline, although now I like it.}{\pos} \\\example{In the past I thought this airline was perfect, now I think it is creepy.}{\neg}} \\
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{Negation}}
& \textbf{\em MFT:} Negated negative should be positive or neutral & 18.8 & 54.2 & 29.4 & 13.2 & 2.6 & \makecell[ml]{\example{The food is not poor.}{\mybox{pos or neutral}} \\\example{It isn't a lousy customer service.}{\mybox{pos or neutral}}} \\ %
\addlinespace
& \textbf{\em MFT:} Negated neutral should still be neutral & 40.4 & 39.6 & 74.2 & 98.4 & 95.4& \makecell[ml]{\example{This aircraft is not private.}{\neutral} \\\example{This is not an international flight.}{\neutral}} \\ %
\addlinespace
& \textbf{\em MFT:} Negation of negative at the end, should be pos. or neut.& 100.0 & 90.4 & 100.0 & 84.8 & 7.2 & \makecell[ml]{\example{I thought the plane would be awful, but it wasn't.}{\mybox{pos or neutral}} \\\example{I thought I would dislike that plane, but I didn't.}{\mybox{pos or neutral}}} \\ %
\addlinespace
& \textbf{\em MFT:} Negated positive with neutral content in the middle & 98.4 & 100.0 & 100.0 & 74.0 & 30.2& \makecell[ml]{\example{I wouldn't say, given it's a Tuesday, that this pilot was great.}{\neg} \\\example{I don't think, given my history with airplanes, that this is an amazing staff.}{\neg}} \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{SRL}}
& \textbf{\em MFT:} Author sentiment is more important than of others & 45.4 & 62.4 & 68.0 & 38.8 & 30.0 & \makecell[ml]{\example{Some people think you are excellent, but I think you are nasty.}{\neg} \\\example{Some people hate you, but I think you are exceptional.}{\pos}} \\
\addlinespace
& \textbf{\em MFT:} Parsing sentiment in (question, ``yes'') form & 9.0 & 57.6 & 20.8 & 3.6 & 3.0& \makecell[ml]{\example{Do I think that airline was exceptional? Yes.}{\neg} \\\example{Do I think that is an awkward customer service? Yes. \neg}{}} \\
\addlinespace
& \textbf{\em MFT:} Parsing sentiment in (question, ``no'') form & 96.8 & 90.8 & 81.6 & 55.4 & 54.8 & \makecell[ml]{\example{Do I think the pilot was fantastic? No.}{\neg} \\\example{Do I think this company is bad? No.}{\mybox{pos or neutral}}} \\

